Last Truck Scheduling for Middle-mile Next-day Delivery Coverage

We consider an e-commerce retailer operating a supply chain that consists of middle- and last-mile transportation, and study its ability to deliver products stored in warehouses within a day from customer's order time. Successful next-day delivery requires inventory availability and timely truck schedules in the middle-mile and in this paper we assume a fixed inventory position and focus on optimizing the middle-mile last truck schedule. We formulate a novel optimization problem which decides the departure of the last truck at each (potential) network connection in order to maximize the number of customer orders that are served with next-day promise. We show that the respective next-day delivery optimization is a combinatorial problem that is NP-hard to approximate within $(1-1/e)opt\approx 0.632opt$, hence every retailer that offers one-day deliveries has to deal with this complexity barrier. We study three variants of the problem motivated by operational constraints that different retailers encounter, and propose solutions schemes tailored to each problem's properties. To that end, we rely on greedy submodular maximization, pipage rounding techniques, and Lagrangian heuristics. The algorithms are scalable, offer worst-case optimality gap guarantees, and evaluated in realistic datasets and network scenarios were found to achieve even near-optimal results.

==> pipage_ob.tex <==
\subsection{Pipage step for $\cP_1^{(\text{ob})}$}
\label{sec:pipage_ob}

In the typical pipage algorithm a step is taken in one dimension, e.g., usually we need to update a vector whose aggregate values needs to satisfy some capacity constraint. In this case, a straightforward approach is to choose two non-integral elements of the vector, say $x_1$ and $x_2$ and perform a symmetric operation where we add and subtract the same value from these elements, i.e.,  $x_1 + \epsilon$ and $x_2 - \epsilon$. This ensures that the constraint is always satisfied. 

In the $\cP_1^{(\text{ob})}$ problem, apart from the constraint that sets all timeslots to 0 after the departure deadline (these variables are already integral so are not considered in the pipage routine anyway) the constraints we need to satisfy are:
\begin{align}
\sum_{t\in\cT} x_{i,j,t}\leq 1, & \quad\forall i \in \cW, \forall j\in\cD, \\
\sum_{j\in\cD} x_{i,j,t} \leq c^{\text{(ob)}}_{i}, & \quad\forall i \in \cW, \forall t\in\cT.
\end{align}
Note that these constraints should be satisfied $\forall i \in \cW$. Therefore, we focus on finding directions for the pipage step that apply feasible updates for a fixed $i$. This implies that we apply the pipage routine for all $i\in\cW$ in parallel.

For a fixed $i$ the proposed pipage routine is a two-step procedure. First we find all the cycles (Section \ref{sec:pipage_ob_cycles}) and in the end we update all the remaining non-cyclic paths (Section \ref{sec:pipage_ob_paths}).



\subsubsection{Cyclic directions}
\label{sec:pipage_ob_cycles}


Consider a fractional solution $\vX(i) \in \cX^{(ob)}$ and a specific destination $j'\in \cD$ and construct $\vZ \in [0,1]^{|\cW|\times |\cT}$ such that $z_{i,t} = x_{i,j',t}$. Below we analyze $\vZ(\ell)$ and provide a way to iterate and produce $\vZ(\ell+1)$. This process repeats for all destinations and yields a pipage step. %For simplicity we drop references to destination $j'$ and iteration $i$, as these are implied.

%Initially we assume that our solution $\vZ$, where $z_{i,t}\in [0,1], \forall i=1,\dots,|\cW|, ~~t=1,\dots,|\cT|$,  has a number of non-integer values, since otherwise we would not need a pipage step. 

\begin{definition}[Graph $G$]
For a solution $\vZ$, the bipartite graph $G(\vZ)$ is given by $G(\vZ)=(U,V,E)$, where $U=\{u_1,\dots,u_{|\cW|}\}$, $V=\{v_1, \dots, v_{|\cT|}\}$ and $E=\{(u_i,v_t): z_{i,t}\in (0,1)\}$. Also, let $\hat{G}(\vZ)$ be its undirected counterpart.
\end{definition}
 
Note that $G(\vZ)$ connects $i$ and $t$ iff $z_{i,t}$ is a fractional value. For example, consider a solution:
\[
\vZ=\left[\begin{array}{ccc}
0.2 & 0.5 & 0.3 \\
0.7 & 0.3 & 0 \\
1 & 0.2 & 0.7
\end{array}\right]
\]
Then  $G(\vZ)$ and $\hat{G}(\vZ)$ are given in (i)-(ii) of Fig.~\ref{fig:graph}.

\begin{figure}[h!]
  \includegraphics[width=\linewidth]{graph}
  \caption{An example: (i) Graph $G(\vZ)$. (ii) Graph $\hat{G}(\vZ)$. (iii) A 4-hop cycle. (iv) A 6-hop cycle.}
  \label{fig:graph}
\end{figure}

A cycle in $\hat{G}(\vZ)$ is an ordered list of links $c=(e_1,\dots,e_k), e_j\in E$, which forms a node sequence $(w_1,\dots, w_k, w_1)$ with the same start and end. Each two successive links share the same node, i.e., if $e_j,e_{j+1}$ are successive links in the cycle, then $e_j=(v_{i-1}, v_i)$ and $e_{j+1}=(v_i, v_{i+1})$. Two examples of cycles are highlighted in Fig.~\ref{fig:graph}(iii)-(iv).

\begin{definition}[Direction $\vY^c$]
Suppose $\hat{G}(\vZ)$ contains a cycle $c$. Then define direction $\vY^c$ as follows:
\begin{equation}\label{eq:conv-dir}
y_{i,t}^c=\left\{\begin{array}{rl}
0 & \text{ if } (i,t), (t,i)\notin c, \\
1 & \text{ if } (i,t)\in c, \\
-1 & \text{ if } (t,i)\in c. 
\end{array}\right.
\end{equation}
\end{definition}

For the examples (iii) and (iv) of the figure we would get:
\[
\vY^1 = \left[\begin{array}{rrr}
1 & -1 & 0 \\
-1 & 1 & 0 \\
0 & 0 & 0
\end{array}\right]
\quad\quad
\vY^2 = \left[\begin{array}{rrr}
1 & 0 & -1 \\
-1 & 1 & 0 \\
0 & -1 & 1
\end{array}\right]
\]


\begin{lemma}\label{lem:zerosum}
The sum of each row and column of $\vY^c$ is 0.
\end{lemma}
\begin{proof}
A cycle in a bipartite graph visits each node an even amount of times $2k$, $k$ entering and $k$ leaving the node. 
Consider node  $t$ of $\hat{G}(\vZ)$, it follows:
\[
\sum_{i=1}^{|\cW|} y_{i,t}^c = \sum_{i: (i,t)\in c} y_{i,t}^c +\sum_{i: (t,i)\in c} y_{i,t}^c = k-k=0.
\]
Similarly
\[
\sum_{t=1}^{|\cT|} y_{i,t}^c = \sum_{t: (i,t)\in c} y_{i,t}^c +\sum_{t: (t,i)\in c} y_{i,t}^c = k-k=0.
\]
\end{proof}

\begin{lemma}\label{lem:pipstep}
There exist small $\epsilon^+,\epsilon^->0$ such that the following hold:
\begin{enumerate}
\item[(i)] Solutions $\vZ+\epsilon^+ \vY^c$ and $\vZ-\epsilon^- \vY^c$ are feasible, i.e., $\vZ+\epsilon^+ \vY^c,\vZ-\epsilon^- \vY^c\in \cX^{(in)}$.
\item[(ii)] Solutions $\vZ+\epsilon^+ \vY^c$ and $\vZ-\epsilon^- \vY^c$ have at least 1 more integer value than $\vZ$. 
\item[(iii)] One of the following is true:
\[
f(\vZ+\epsilon^+ \vY^c)\geq f(\vZ) \quad\text{ or }\quad  f(\vZ-\epsilon^- \vY^c)\geq f(\vZ).
\] 
\end{enumerate}
\end{lemma}
\begin{proof} \todo{Improve the proof}
For (i), we show that all constraints in $\cX^{(in)}$ are satisfied using Lemma~\ref{lem:zerosum} that states that the direction $\vY^c$ has sum of rows and columns zero. First, for the side constraints, we combine  the fact that $x\in\mathcal{P}$ with Claim~\ref{cl:1}.  From the first, we have that $\sum_{i=1}^Ix_{ij}=1, ~\forall j$. Then
\[
\sum_{i=1}^I(x_{ij}+\epsilon^+ y_{ij}) = \sum_{i=1}^Ix_{ij}+\epsilon^+\sum_{i=1}^I y_{ij} = 1+0=1,~\forall j,
\]
where $\sum_{i=1}^I y_{ij}=0$ is due to lemma~\ref{}. The same is true for $x-\epsilon^- y$, as well as for the other side constraint. It remains to show that there exists $\epsilon^+>0$ sufficiently small such that the elements of $x+\epsilon^+ y$ take values in $[0,1]$. Note, that every link $(i,j)$ in $c$ is also a link in $\hat{G}(x)$, hence corresponds to a fractional variable $x_{ij}\in (0,1)$. Therefore, there is $\epsilon_{ij}>0$ such that $x_{ij}\pm \epsilon_{ij}\in [0,1]$.

For (ii), we use the fact that every link $(i,j)$ in $c$ is also a link in $\hat{G}(x)$, hence corresponds to a fractional variable $x_{ij}\in (0,1)$. Therefore, there is $\epsilon_{ij}>0$ such that $x_{ij}+- \epsilon_{ij}\in [0,1]$.

For (iii), it suffices to show that $g(\vX)$ is convex in the direction $\vY$, i.e., $g(\vX + \epsilon \vY)$ is convex with respect to $\epsilon$
\end{proof}



\begin{algorithm}
\caption{\texttt{Pipage-step}}\label{alg:pipage}
\begin{algorithmic}
\State Read input $\vX$ 
\For{$j=1:|\cD|$}
	\State $z_{i,t} \gets x_{i,j,t}, \quad \forall i\in\cW, t\in\cT$
	\State Build $\hat{G}(\vZ)$ by opening link $(u_i,v_t)$ iff $z_{i,t}\in (0,1)$
	\State $c \gets \texttt{Cycle}(G(\vZ))$
	\State Compute direction $\vY^c$ using \eqref{eq:conv-dir}
	\State $\epsilon^+ \gets$ \todo{}
	\State $\epsilon^- \gets$ \todo{}
	\State $\vZ \gets \arg\max\{f(\vZ+\epsilon^+ \vY^c),f(\vZ-\epsilon^- \vY^c)\}$
	\State $x_{i,j,t} \gets z_{i,t}, \quad \forall i\in\cW, t\in\cT$
\EndFor
% \Ensure $y = x^n$
% \State $y \gets 1$
% \State $X \gets x$
% \State $N \gets n$
% \While{$N \neq 0$}
% \If{$N$ is even}
%     \State $X \gets X \times X$
%     \State $N \gets \frac{N}{2}$  \Comment{This is a comment}
% \ElsIf{$N$ is odd}
%     \State $y \gets y \times X$
%     \State $N \gets N - 1$
% \EndIf
% \EndWhile
\end{algorithmic}
\end{algorithm}


\subsubsection{Non-cyclic directions}
\label{sec:pipage_ob_paths}

bla
